Black Hole - Neutron Star Binary Mergers: The Imprint of Tidal Deformations and Debris

The increase in the sensitivity of gravitational wave interferometers will bring additional detections of binary black hole and double neutron star mergers. It will also very likely add many merger events of black hole - neutron star binaries. Distinguishing mixed binaries from binary black holes mergers for high mass ratios could be challenging because in this situation the neutron star coalesces with the black hole without experiencing significant disruption. To investigate the transition of mixed binary mergers into those behaving more like binary black hole coalescences, we present results from merger simulations for different mass ratios. We show how the degree of deformation and disruption of the neutron star impacts the inspiral and merger dynamics, the properties of the final black hole, the accretion disk formed from the circularization of the tidal debris, the gravitational waves, and the strain spectrum and mismatches. The results also show the effectiveness of the initial data method that generalizes the Bowen-York initial data for black hole punctures to the case of binaries with neutron star companions.

==> defs.tex <==
\newcommand{\amp}[0]{\&}
\newcommand{\KMS}{\mbox{km s}^{-1}\,}    
\newcommand{\peter}[0]{M\'esz\'aros}
\newcommand{\Ms}{\ifmmode{\textrm{M}_\odot}\else{$M_\odot$}\fi}
\newcommand{\msun}[0]{{\text{M}_{\odot}}}
\newcommand{\eod}[0]{Education, Outreach and Diversity}
\newcommand{\ehrd}[0]{Education and Human Resource Development}
\newcommand{\gwnet}[0]{\gsfc\ Astroparticle Physics Laboratory and Gravitational Astrophysics Laboratory, \ornl\ Theoretical Astrophysics Group, \cgwa, University of T\"ubingen Institute for \tat, and the German \sfb}
\newcommand{\nasa}[0]{NASA}
\newcommand{\nsf}[0]{NSF}
\newcommand{\icecube}[0]{IceCube}
\newcommand{\epo}[0]{Deputy \& Outreach}
\newacronym{\cra}{CRA}{Center for Relativistic Astrophysics}
\newacronym{\ma}{MA}{Major Activity}
\newacronym{\cgwp}{CGWP}{Center for Gravitational Wave Physics}
\newacronym{\hpc}{HPC}{high performance computing}
\newacronym{\tat}{TAT}{Theoretische Astrophysik T\"ubingen}
\newacronym{\gsfc}{GSFC}{Goddard Space Flight Center}
\newacronym{\ornl}{ORNL}{Oak Ridge National Laboratory}
\newacronym{\lisa}{LISA}{Laser Interferometer Space Antenna}
\newacronym{\hawc}{HAWC}{High-Altitude Water Cherenkov Observatory}
\newacronym{\cta}{CTA}{Cherenkov Telescope Array}
\newacronym{\ska}{SKA}{Square Kilometer Array}
\newacronym{\lsst}{LSST}{Large Synoptic Survey Telescope}
\newacronym{\doe}{DOE}{Department of Energy}
\newacronym{\esa}{ESA}{European Space Agency}
\newacronym{\ligo}{LIGO}{Laser Interferometer Gravitational-wave
  Observatory} 
\newacronym{\lsc}{LSC}{LIGO Scientific Collaboration}
\newacronym{\Caltech}{Caltech}{California Institute of Technology}
\newacronym{\PFC}{PFC}{Physics Frontier Center}
\newacronym{\pfc}{PFC}{Physics Frontier Center}
\newacronym{\EOD}{EOD}{Education, Outreach and Diversity}
\newacronym{\MIT}{MIT}{Massachusetts Institute of Technology}
\newacronym{\sph}{SPH}{smooth particle hydrodynamics}
\newacronym{\tsi}{TSI}{Terascale Supernova Initiative}
\newacronym{\wmap}{WMAP}{the Wilkinson Microwave Anisotropy Probe}
\newacronym{\decigo}{DECIGO}{the Deci-Hertz Interferometric
  Gravitational-wave Observatory} 
\newacronym{\cmbr}{CMBR}{cosmic microwave background}
\newacronym{\ibbh}{IBBH}{intermediate binary black hole}
\newacronym{\bdj}{BDJ}{Brans-Dicke-Jordan}
\newacronym{\bbo}{BBO}{Big Bang Observer}
\newacronym{\decigo}{DECIGO}{Deci-Hertz Gravitational-Wave Observatory}
\newacronym{\cgwa}{UTB/CGWA}{University of Texas (Brownsville) Center for Gravitational Wave Astronomy}
\newacronym{\wiser}{WISER}{Women In Science and Engineering Research}
\newacronym{\mure}{MURE}{Minority Undergraduate Research Experience}
\newacronym{\igc}{IGC}{Institute for Gravitation and the Cosmos}
\newacronym{\sfb}{SFB/TR7}{Sonderforschungsbereich Transgerio 7, Gravitational Wave Astronomy Methods, Sources \& Observations}
\newacronym{\inst}{CMA}{Center for Multi-messenger Astrophysics}
\newacronym{\eos}{EOS}{equation of state}
\newacronym{\osg}{OSG}{Open Science Grid}
\newacronym{\gt}{GaTech}{Georgia Institute of Technology}
\newacronym{\mda}{MDA}{Multi-messenger Data Archive}
\newacronym{\ceismc}{CEISMC}{Center for Education Integrating Science, Mathematics, and Computing}
\newacronym{\mda}{MDA}{Multi-messenger Data Archiving}


\newcommand{\maa}[0]{The Messengers: Photons, Particles and Gravitational Waves}
\newcommand{\mab}[0]{The Backbone: Data, Computing and Instrumentation}
\newcommand{\mac}[0]{Advancing the Multi-Messenger Community}

\def\emri#1{Extreme Mass-Ratio Inspiral#1 (EMRI#1)\gdef\emri{EMRI}}
\def\gw#1{gravitational wave#1 (GW#1)\gdef\gw{GW}}
\def\bh#1{black hole#1
  (BH#1)\gdef\bh{BH}}
\def\ns#1{neutron star#1
  (NS#1)\gdef\ns{NS}}
\def\grb#1{Gamma-Ray Burst#1
  (GRB#1)\gdef\grb{GRB}}
\def\imbh#1{intermediate mass black hole#1
  (IMBH#1)\gdef\imbh{IMBH}}
\def\smbh#1{supermassive black hole#1
  (SMBH#1)\gdef\smbh{SMBH}}
\def\ulx#1{ultra-luminous x-ray source#1 (ULX#1)\gdef\ulx{ULX}}
\def\lmxbs{low-mass x-ray Binaries
  (LMXBs)\gdef\lmxbs{LMXBs}\gdef\lmxb{LMXB}} 
\def\lmxb{low-mass x-ray Binary
  (LMXB)\gdef\lmxbs{LMXBs}\gdef\lmxb{LMXB}} 
\def\emrb{extreme mass-ratio binary
  (EMRB)\gdef\emrb{(EMRB}\gdef\emrbs{EMRBs}} 
\def\emrbs{extreme mass-ratio binaries
  (EMRBs)\gdef\emrb{(EMRB}\gdef\emrbs{EMRBs}} 

\def\aj{Astronomical Journal }                 % Astronomical Journal
\def\apj{Astrophysical Journal }                % Astrophysical Journal
\def\apjl{Astrophysical Journal Letters}             % Astrophysical Journal, Letters
\def\pasj{PASJ }
\def\apjs{ApJS }              % Astrophysical Journal, Supplement
\def\mnras{MNRAS }            % Monthly Notices of the RAS
\def\prd{Physical Review D }       % Physical Review D
\def\prl{Physical Review Letters }    % Physical Review Letters
\def\cqg{Classical \& Quantum Gravity }%Classical and Quantum Gravity
\def\nat{Nature}              % Nature
\def\physrep{Physics Reports} % Physics Reports
\def\na{New Astronomy}		% New Astronomy
\def\aapr{Astronomy \& Astrophysics Reviews}	%Astronomy and Astrophysics Reviews
\def\araa{Annual Reviews of Astronomy \& Astrophysics} 
\def\aap{Astronomy \& Astrophysics}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "body"
%%% End: 

